A Unified View of Abstract Visual Reasoning Problems

The field of Abstract Visual Reasoning (AVR) encompasses a wide range of problems, many of which are inspired by human IQ tests. The variety of AVR tasks has resulted in state-of-the-art AVR methods being task-specific approaches. Furthermore, contemporary methods consider each AVR problem instance not as a whole, but in the form of a set of individual panels with particular locations and roles (context vs. answer panels) pre-assigned according to the task-specific arrangements. While these highly specialized approaches have recently led to significant progress in solving particular AVR tasks, considering each task in isolation hinders the development of universal learning systems in this domain. In this paper, we introduce a unified view of AVR tasks, where each problem instance is rendered as a single image, with no a priori assumptions about the number of panels, their location, or role. The main advantage of the proposed unified view is the ability to develop universal learning models applicable to various AVR tasks. What is more, the proposed approach inherently facilitates transfer learning in the AVR domain, as various types of problems share a common representation. The experiments conducted on four AVR datasets with Raven's Progressive Matrices and Visual Analogy Problems, and one real-world visual analogy dataset show that the proposed unified representation of AVR tasks poses a challenge to state-of-the-art Deep Learning (DL) AVR models and, more broadly, contemporary DL image recognition methods. In order to address this challenge, we introduce the Unified Model for Abstract Visual Reasoning (UMAVR) capable of dealing with various types of AVR problems in a unified manner. UMAVR outperforms existing AVR methods in selected single-task learning experiments, and demonstrates effective knowledge reuse in transfer learning and curriculum learning setups.

==> sections/figures/approach.tex <==
\definecolor{encoder}{HTML}{91BFDB}

\newcommand{\imagedir}{images/rpms}
\newcommand{\rpmid}{raven_rpm_in_center_single_out_center_single_train_1525}
\newcommand{\patch}[2]{\includegraphics[width=7pt]{\imagedir/\rpmid/patches/patch_#1_#2}}
\newcommand{\panel}[2]{\includegraphics[width=0.045\textwidth]{\imagedir/\rpmid/panels/#1_#2}}

\newcommand{\smallunit}{4pt}
\newcommand{\unit}{8pt}

\tikzstyle{panel} = [thick, rectangle, draw=black, inner sep=0]
\tikzstyle{background} = [draw, fill=black!5, rounded corners=5pt, dashed, inner sep=0]
\tikzstyle{vector} = [rectangle, draw=black, minimum width=5*\unit, minimum height=\smallunit]
\tikzstyle{encoder} = [rectangle, rounded corners, text centered, draw=black, fill=encoder, font=\bfseries]
\tikzstyle{arrow} = [thick,->,>={Latex[scale=1]}]
\tikzstyle{unit} = [minimum size=\unit]

\begin{figure}[t]
    \centering
    \begin{tikzpicture}
        % split RPM
        \begin{scope}[node distance=-6pt]
            \node (p_0_0) {\patch{0}{0}};

            \foreach \i in {1,...,18} {
                \pgfmathtruncatemacro{\prev}{\i - 1}
                \node (p_\i_0) [below=of p_\prev_0] {\patch{\i}{0}};
            }

            \foreach \i in {0,...,18} {
                \foreach \j in {1,...,9} {
                    \pgfmathtruncatemacro{\prev}{\j - 1}
                    \node (p_\i_\j) [right=of p_\i_\prev] {\patch{\i}{\j}};
                }
            }
        \end{scope}
        \begin{scope}[on background layer]
            \node (bg_split_rpm) [fit={(p_0_0) (p_18_9)}, background] {};
        \end{scope}

        % unified RPM
        \node (rpm) [left=of bg_split_rpm, xshift=-7pt] {
            \includegraphics[width=0.18\textwidth]{\imagedir/\rpmid/rpm}
        };
        \begin{scope}[on background layer]
            \node (bg_rpm) [fit={(rpm.north west) (rpm.south east)}, background] {};
        \end{scope}
        \node (rpm_math) [above=of rpm.north, yshift=-25pt] {$\bm{\chi}^t$};

        % panels
        \begin{scope}[node distance=3pt]
            \node (p0) [left=of bg_rpm.north west, xshift=-0.1\textwidth, yshift=-15pt] {\panel{context}{0}};
            \node (p1) [below=of p0] {\panel{context}{1}};
            \node (pn) [left=of bg_rpm.south west, xshift=-0.1\textwidth, yshift=15pt] {\panel{answer}{7}};
        \end{scope}
        \begin{scope}[on background layer]
            \node (bg_p0) [fit={(p0.north west) (p0.south east)}, background] {};
            \node (bg_p1) [fit={(p1.north west) (p1.south east)}, background] {};
            \node (bg_pn) [fit={(pn.north west) (pn.south east)}, background] {};
        \end{scope}
        \node (brace_top) [inner sep=0] at (bg_pn.south east |- bg_p0.north east) {};
        \node (brace_center) at ($ (brace_top)!0.5!(bg_pn.south east) $) {};
        \draw [decoration={brace,raise=0.2cm}, decorate, line width=1.25pt] (brace_top) node {} -- (bg_pn.south east);
        \draw[arrow] ($ (brace_center.east) + (0.15cm, 0) $) -- node (merge) [midway, above] {Merge} (bg_rpm);
        \node (renderer) [below=of merge, yshift=25pt] {$\mathcal{R}(\cdot)$};
        \draw [thick, loosely dotted] ($ (p1.south) + (0, -0.2cm) $) -- ($ (pn.north) + (0, 0.2cm) $);
        \node (panels_math) [above=of p0.north, yshift=-25pt] {$\{\bm{x}_j^t\}$};

        % patches
        \begin{scope}[node distance=0.3cm]
            \node (q0) [right=of p_0_9, xshift=1cm] {\patch{0}{0}};
            \node (q1) [below=of q0] {\patch{0}{1}};
            \node (q2) [below=of q1] {\patch{0}{2}};
            \node (qn) [right=of p_18_9, xshift=1cm] {\patch{18}{9}};
        \end{scope}
        \begin{scope}[on background layer]
            \foreach \i in {0,...,2} {
                \node (bg_q\i) [fit={(q\i.north west) (q\i.south east)}, background] {};
            }
            \node (bg_qn) [fit={(qn.north west) (qn.south east)}, background] {};
        \end{scope}
        \draw [thick, loosely dotted] ($ (bg_q2.south) + (0, -0.2cm) $) -- ($ (bg_qn.north) + (0, 0.2cm) $);
        \node (patches_math) [above=of q0.north, yshift=-25pt] {$\{\bm{p}_{k,l}\}$};

        % patch encoder
        \begin{scope}[node distance=-0.15cm]
            \node (pe0) [unit, right=of q0, xshift=0.6cm, inner sep=12pt] {};
            \node (pe1) [unit, right=of q1, xshift=0.6cm, inner sep=12pt] {};
            \node (pe2) [unit, right=of q2, xshift=0.6cm, inner sep=12pt] {};
            \node (pen) [unit, right=of qn, xshift=0.6cm, inner sep=12pt] {};
        \end{scope}
        \node (patch_encoder) [fit={(pe0) (pen)}, encoder, inner sep=0] {};
        \node [align=center, rotate=90] at (patch_encoder.center) {Patch-based model $\mathcal{F}(\cdot)$};

        \draw[arrow] (bg_rpm.east) -- node [midway, above] {Split} (bg_split_rpm.west);

        \draw [c0, arrow] ($ (p_0_0.north) + (0, -0.1cm) $)
            to[out=90, in=180] ($ (p_0_4.north) + (0, 0.6cm) $)
            to[out=0, in=180] ($ (p_0_8.north) + (0, 0.6cm) $)
            to[out=0, in=120] ($ (q0.west) + (-0.7cm, 0.3cm) $)
            to[out=300, in=180] (bg_q0.west);

        \draw [c1, arrow] ($ (p_0_1.north) + (0, -0.1cm) $)
            to[out=90, in=180] ($ (p_0_4.north) + (0, 0.4cm) $)
            to[out=0, in=180] ($ (p_0_8.north) + (0, 0.4cm) $)
            to[out=0, in=120] ($ (q1.west) + (-0.7cm, 0.5cm) $)
            to[out=300, in=180] (bg_q1.west);

        \draw [c2, arrow] ($ (p_0_2.north) + (0, -0.1cm) $)
            to[out=90, in=180] ($ (p_0_4.north) + (0, 0.2cm) $)
            to[out=0, in=180] ($ (p_0_8.north) + (0, 0.2cm) $)
            to[out=0, in=120] ($ (q2.west) + (-0.7cm, 0.5cm) $)
            to[out=300, in=180] (bg_q2.west);

        \draw [c3, arrow] ($ (p_18_9.east) + (-0.1cm, 0) $) -- (bg_qn.west);

        \draw [c0, arrow] (bg_q0.east) -- (pe0.west);
        \draw [c1, arrow] (bg_q1.east) -- (pe1.west);
        \draw [c2, arrow] (bg_q2.east) -- (pe2.west);
        \draw [c3, arrow] (bg_qn.east) -- (pen.west);

    \end{tikzpicture}
    \caption{
    \textbf{Unified patch-based AVR.}
    In the unified perspective, single matrix panels $\{\bm{x}_j^t\}_{j=1}^{P_t}$ are merged by a rendering module $\mathcal{R}$ into a unified image $\bm{\chi}^t$.
    To facilitate discovery of low- and high-level patterns, the unified image is split into a grid of patches $\{\{\bm{p}_{k,l}\}_{k=1}^R\}_{l=1}^C$.
    These patches form the input to a predictive patch-based model $\mathcal{F}$.
    }
    \label{fig:approach}
\end{figure}


==> sections/figures/embeddings-pgm-1x4.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.98\textwidth]{images/embeddings-pgm-1x4.pdf}
    \caption{
    \textbf{PGM embeddings.}
    The embeddings of PGM matrices ($n_a=2$) from the test split, visualized with t-SNE~\cite{van2008visualizing}.
    }
    \label{fig:embeddings-pgm-1x4}
\end{figure}


==> sections/figures/embeddings-raven-1x4.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.98\textwidth]{images/embeddings-raven-1x4.pdf}
    \caption{
    \textbf{I-RAVEN embeddings.}
    The embeddings of I-RAVEN matrices ($n_a=2$) from the test split, visualized with t-SNE~\cite{van2008visualizing}.
    }
    \label{fig:embeddings-raven-1x4}
\end{figure}


==> sections/figures/embeddings-vap.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.98\textwidth]{images/embeddings-vap.pdf}
    \caption{
    \textbf{Embeddings.}
    The embeddings of VAP matrices ($n_a=2$) from the test split, visualized with t-SNE~\cite{van2008visualizing}.
    }
    \label{fig:embeddings-vap}
\end{figure}

